JaxNet: Scalable Blockchain Network

Today's world is organized based on merit and value. A single global currency that's decentralized is needed for a global economy. Bitcoin is a partial solution to this need, however it suffers from scalability problems which prevent it from being mass-adopted. Also, the deflationary nature of bitcoin motivates people to hoard and speculate on them instead of using them for day to day transactions. We propose a scalable, decentralized cryptocurrency that is based on Proof of Work. The solution involves having parallel chains in a closed network using a mechanism which rewards miners proportional to their effort in maintaining the network. The proposed design introduces a novel approach for solving the scalability problem in the blockchain network based on merged mining.

==> 3_Architecture/Transactions.tex <==
\subsection{Transactions}

==> 6_Appendices/RecentPaperOnEfficiency.tex <==
\subsection{Recent paper}

In the recent paper by Yo-Der Song and Tomaso Aste \cite{song2020cost}

==> AbstractWP.tex <==
Today’s world is organized based on merit and value. A single global currency that’s decentralized is needed for a global economy. Bitcoin is a partial solution to this need, however it suffers from scalability problems which prevent it from being mass-adopted. Also, the deflationary nature of bitcoin motivates people to hoard and speculate on them instead of using them for day to day transactions. We propose an inflationary, scalable, decentralized cryptocurrency that is based on proof of work. The solution involves having parallel chains in a closed network using a reward mechanism based on CPU power spent.

==> draft.tex <==
Simulation of the Bitcoin Network Considering
Compact Block Relay and Internet Improvements
\cite{nagayama2019simulation}

... block propagation delay in the Bitcoin network has been shortened in recent years.

The experimental results reveal that the block propagation delay is reduced by 64.5\% for the 50th percentile and 63.7\% for the 90th percentile due to Internet improvements, and by 90.1\% for the 90th percentile and by 87.6\% for the 90th percentile due to compact block relay.

%%%%%%%%%%%%%%%%%%%%

An Equilibrium Valuation of Bitcoin
and Decentralized Network Assets 
\cite{pagnotta2018equilibrium}

%%%%%%%%%%%%%%%%%%%%

Merged mining allows a miner to mine for more than one block chain at the same time. The benefit is that every hash the miner does contributes to the total hash rate of both (all) currencies, and as a result they are all more secure.

%%%%%%%%%%%%%%%%%%%%

All that Glitters is not Bitcoin-Unveiling the Centralized Nature of the BTC (IP) Network
\cite{ben2020all}

In BTC, each node keeps a list of up
to 2,500 peer addresses of tried and new connections to its neighbors [1].

and current BTC full blockchain accounts for about 218 GB.

 Current aggregated daily
mining reward is close to 15 million USD.

The crawler discovers more than 200,000 BTC IPs, with a total of 9,673 active nodes – recall that this number does not reflect the actual number of BTC users/wallets, which are better captured through analysis of the BTC transactions [2]

Despite such a western concentration of active nodes, it is impressive to see that the far majority of BTC mining activity actually occurs in China. As we explained before, by using the signatures provided by the miners when producing a new block, we identify the main mining pools, and observe that more than 70\% of the BTC mining activity is controlled by major Chinese mining pools – we dig deeper into this next.

%%%%%%%%%

Cryptocurrency networks: A new P2P paradigm \cite{delgado2018cryptocurrency}

Peers participating in the network store some data about the blockchain. However, the exact data they store dier largely, from a few megabytes to dozens of gigabytes. Full blockchain peers store a complete and up-to-date version of the blockchain (on September 2016, the total size of block Full blockchain Pruned blockchain Headers only Miners Validation and relaying Wallet Others: DNS, block explorer, exchange service, mixing service, and so on. Listening peer Nonlistening peer Bitcoin Getblocktemplate Stratum Corallo’s fast relay network Falcon FIBRE FLARE Bitcoin node Blockchain knowledge Functionality Connectivity Protocol implemented Figure 3: Bitcoin node classication. 4 Mobile Information Systems headers and transactions consists of 80 GB of data). Pruned blockchain peers store an up-to-date version of the blockchain with complete blockchain data for at least the last 2 days (the number of days for which to store complete blockchain data can be tuned by users. Pruned mode is estimated to reduce disk usage to around 2 GB [7]). Although only storing complete blockchain data for a few days, pruned nodes are able to securely validate transactions because they indeed store the required information from their previous history of the blockchain, that is, metadata about all known blocks and the UTXO set. Simplified payment verification (SPV) clients have an up-to-date version of the blockchain headers (a block header is an 80-byte structure. On September 2016, the Bitcoin blockchain has 432,000 blocks, thus needing around 33 MB of the disk space). Additionally, SPV clients may store transaction data from some transactions of interest. SPV clients are usually deployed in mobile devices such as smartphones, where having the full blockchain is generally unaffordable.



==> tikz_pic/SCchain.tex <==
\begin{figure}[ht!]
	\begin{center}
		\resizebox{0.7\textwidth}{!}{
			\begin{tikzpicture}

\node (CMCBlockN)[labelnode, draw=black!30, outer color=orange!5, label={[black]90:{\scalebox{2}{BC Block Header $\#N-1$}}}] at (0,0)
{Block Header $\#N$};
\node (CMCBlockN-1) at (-10,0)
{Block Header $\#N-1$};
\node (CMCBlockN+1) at (+10,0)
{Block Header $\#N+1$};			
			\end{tikzpicture}
		}
		\vspace*{3pt}
		%\captionsetup{labelformat=empty}
		\caption{\textbf{Shard Chain in JaxNet}} \label{SCchain}
    \end{center}
\end{figure}
